Meta-tuning Loss Functions and Data Augmentation for Few-shot Object Detection

Few-shot object detection, the problem of modelling novel object detection categories with few training instances, is an emerging topic in the area of few-shot learning and object detection. Contemporary techniques can be divided into two groups: fine-tuning based and meta-learning based approaches. While meta-learning approaches aim to learn dedicated meta-models for mapping samples to novel class models, fine-tuning approaches tackle few-shot detection in a simpler manner, by adapting the detection model to novel classes through gradient based optimization. Despite their simplicity, fine-tuning based approaches typically yield competitive detection results. Based on this observation, we focus on the role of loss functions and augmentations as the force driving the fine-tuning process, and propose to tune their dynamics through meta-learning principles. The proposed training scheme, therefore, allows learning inductive biases that can boost few-shot detection, while keeping the advantages of fine-tuning based approaches. In addition, the proposed approach yields interpretable loss functions, as opposed to highly parametric and complex few-shot meta-models. The experimental results highlight the merits of the proposed scheme, with significant improvements over the strong fine-tuning based few-shot detection baselines on benchmark Pascal VOC and MS-COCO datasets, in terms of both standard and generalized few-shot performance metrics.

==> coco_baseline_vs_metatune.tex <==


\begin{table}[t!]
\caption{\textcolor{red}{Evaluation of meta-tuning variants over MPSR~\cite{wu2020multi}  and TFA~\cite{wang2020frustratingly} on the MS-COCO dataset.}}
\label{coco_baseline_vs_metatune}
\begin{center}
\begin{scriptsize}
\begin{tabular}{c|cc|cc}
\toprule
                               & \multicolumn{2}{c|}{Novel Classes}                & \multicolumn{2}{c}{All Classes (HM)} \\
\multirow{-2}{*}{Method/Shots} & 10-shot                            & 30-shot     & 10-shot        & 30-shot        \\ \midrule
MPSR                           & 9.1                                & 13.7        & 11.5           & 15.0           \\
MPSR+Meta-Static                           &  10.1 & 14.8 & 12.7    & 16.4    \\
MPSR+Meta-Dynamic                         & 11.9                        & 14.9& 14.3    & 16.6   \\
MPSR+Meta-ScaledDynamic                        & \textbf{12.3}                        & \textbf{15.0}& \textbf{14.4}    & \textbf{16.7}   \\ \midrule
TFA                            & 10.0                               & 13.7        & 15.6           & 19.8           \\
TFA+Meta-Static                   & 10.4                        & 14.4 & 16.1     & 20.6
\\
TFA+Meta-Dynamic                   & 10.7                        & 14.7 & 16.3     & 20.8
\\
TFA+Meta-ScaledDynamic                   & \textbf{10.9}                        & \textbf{15.0} & \textbf{16.4}     & \textbf{21.0}
\\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}


==> pascal_tl.tex <==
%!TEX root=FSOD-NeurIPS22.tex

\begin{table*}
    \caption{FSOD results on the Pascal VOC dataset with base classes. The best and the second-best results are marked with \textcolor{red}{red} and \textcolor{blue}{blue}. MPSR+MetaTuneS and MPSR+MetaTuneD represent meta-tuning results. FT represent the fine-tuning based methods.}
    %methods that express the hyperparameters of the classification loss function with a single distribution, and with a time-dependent polynomial function. FT represent the fine-tuning based methods.}
\label{pascal_novel_tl}
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc|ccccc|ccccc|ccccc}
\toprule
\multicolumn{2}{c|}{}                      & \multicolumn{5}{c|}{Novel Set 1}                                                                                                                                                                 & \multicolumn{5}{c|}{Novel Set 2}                                                                                                                                                                 & \multicolumn{5}{c}{Novel Set 3}                                                                                                                                                                  \\
\multicolumn{2}{c|}{\multirow{-2}{*}{Method/Shot}} & 1                                    & 2                                    & 3                                    & 5                                    & 10                                   & 1                                    & 2                                    & 3                                    & 5                                    & 10                                   & 1                                    & 2                                    & 3                                    & 5                                    & 10                                   \\ \midrule
                         & FRCN~\cite{wang2020frustratingly}    & 15.2                                 & 20.3                                 & 29.0                                 & 25.5                                 & 28.7                                 & 13.4                                 & 20.6                                 & 28.6                                 & 32.4                                 & 38.8                                 & 19.6                                 & 20.8                                 & 28.7                                 & 42.2                                 & 42.1                                 \\
                         & TFA-fc~\cite{wang2020frustratingly}    & 36.8                                 & 29.1                                 & 43.6                                 & \textcolor{red}{ \textbf{55.7}} & 57.0                                 & 18.2                                 & 29.0                                 & 33.4                                 & 35.5                                 & 39.0                                 & 27.7                                 & 33.6                                 & 42.5                                 & 48.7                                 & 50.2 \\
                         & TFA-cos~\cite{wang2020frustratingly}   &  39.8         & 36.1                                 & 44.7                                 & \textcolor{red}{ \textbf{55.7}} & 56.0                                 & 23.5                                 & 26.9                                 & 34.1                                 & 35.1                                 & 39.1                                 & 30.8                                 & 34.8                                 & 42.8                                 & \textcolor{blue}{ \textbf{49.5}} & 49.8                                 \\
                         & MPSR~\cite{wu2020multi}            & 37.2                                 & 43.6                                 & 50.9                                 & 53.7                                 & 60.2                                 & 24.8                                 & 28.1                                 & 38.0                                 & 39.8 &  45.9                               & 37.3                                 & 40.0 & 43.9 & 47.8                                 & 50.1 \\
                         & Ret. R-CNN~\cite{fan2021generalized}      & \textcolor{blue}{ \textbf{42.4}} & 45.8                                 & 45.9                                 & 53.7                                 & 56.1                                 & 21.7                                 & 27.8                                 & 35.2                                 & 37.0                                 & 40.3                                 & 30.2                                 & 37.6                                 & 43.0                                 & \textcolor{red}{ \textbf{49.7}} & 50.1 \\
                         & TFA+H~\cite{zhang2021hallucination}         & \textcolor{red}{ \textbf{45.1}} & 44.0                                 & 44.7                                 & 55.0 & 55.9                                 & 23.2                                 & 27.5                                 & 35.1                                 & 34.9                                 & 39.0                                 & 30.5                                 & 35.1                                 & 41.4                                 & 49.0          & 49.3          \\
\multirow{-7}{*}{FT}     & FSCE~\cite{sun2021fsce}            & 37.6                                 & 44.7                                 & 46.9                                 & 52.2                                 & 60.3                                 & 24.5                                 & 30.1                                 & 38.2                                 & 40.4                                 & 45.9                                 & 25.4                                 & 34.2                                 & 42.3                                 & 48.7                                 & \textcolor{blue}{ \textbf{50.3}}                                 \\ \midrule
                         & MPSR+MetaTuneS             & 36.7                                 & 47.0 & \textcolor{blue}{ \textbf{52.1}} & 53.8                                 & \textcolor{blue}{ \textbf{60.8}} & 25.3 & 31.6 & 38.4 & \textcolor{red}{ \textbf{40.8}} & \textcolor{red}{ \textbf{46.9}} & \textcolor{blue}{ \textbf{38.3}} & 39.7                                 & \textcolor{blue}{ \textbf{44.8}} & 47.2                                 & 50.1 \\
                                                  & MPSR+MetaTuneD            & 40.4                                & \textcolor{blue}{ \textbf{47.5}} & 51.9 &  54.9          & 60.5 & \textcolor{blue}{ \textbf{25.6}} & \textcolor{blue}{ \textbf{31.7}} & \textcolor{blue}{ \textbf{38.5}} & \textcolor{blue}{ \textbf{40.6}} & 46.7 & 37.6 & \textcolor{blue}{ \textbf{40.2}} & 44.7 & 49.1                                 & \textcolor{blue}{ \textbf{50.3}} \\
\multirow{-3}{*}{Ours}     & MPSR+MetaTuneD+s            & 41.5                                & \textcolor{red}{ \textbf{47.9}} & \textcolor{red}{ \textbf{52.7}} &  \textcolor{blue}{ \textbf{55.4}}          & \textcolor{red}{ \textbf{60.9}} & \textcolor{red}{ \textbf{25.7}} & \textcolor{red}{ \textbf{32.2}} & \textcolor{red}{ \textbf{38.9}} & \textcolor{red}{ \textbf{40.8}} & \textcolor{blue}{ \textbf{46.8}} & \textcolor{red}{ \textbf{38.5}} & \textcolor{red}{ \textbf{40.9}} & \textcolor{red}{ \textbf{45.9}} & 49.0                                 & \textcolor{red}{ \textbf{51.0}}\\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}

\end{table*}

